Incremental Cross-view Mutual Distillation for Self-supervised Medical CT Synthesis

Due to the constraints of the imaging device and high cost in operation time, computer tomography (CT) scans are usually acquired with low intra-slice resolution. Improving the intra-slice resolution is beneficial to the disease diagnosis for both human experts and computer-aided systems. To this end, this paper builds a novel medical slice synthesis to increase the between-slice resolution. Considering that the ground-truth intermediate medical slices are always absent in clinical practice, we introduce the incremental cross-view mutual distillation strategy to accomplish this task in the self-supervised learning manner. Specifically, we model this problem from three different views: slice-wise interpolation from axial view and pixel-wise interpolation from coronal and sagittal views. Under this circumstance, the models learned from different views can distill valuable knowledge to guide the learning processes of each other. We can repeat this process to make the models synthesize intermediate slice data with increasing inter-slice resolution. To demonstrate the effectiveness of the proposed approach, we conduct comprehensive experiments on a large-scale CT dataset. Quantitative and qualitative comparison results show that our method outperforms state-of-the-art algorithms by clear margins.

==> tables/tab-gamma.tex <==
\begin{table}[t]
\caption{Performance of using different values for $\gamma$ on the CT dataset. All algorithms are validated under the $4\times$ interpolation setting. %Only the axial view interpolation model is used for testing.
}
\label{tab:gamma}
\centering
\setlength{\tabcolsep}{3.5mm}{
    \begin{tabular}{c|c|c|c|c}
        \toprule
        $\gamma$(\%)  & 10     & 25      & 50     & 100 \\ \midrule
        PSNR      &40.32   & 40.91   &40.73        &40.46      \\ \midrule
        SSIM$_a$  &0.9312  &0.9397   &0.9376    &0.9341      \\ 
        \bottomrule
    \end{tabular}
}
\end{table}
